Yin and Yang: Balancing and Answering Binary Visual Questions

The complex compositional structure of language makes problems at the intersection of vision and language challenging. But language also provides a strong prior that can result in good superficial performance, without the underlying models truly understanding the visual content. This can hinder progress in pushing state of art in the computer vision aspects of multi-modal AI. In this paper, we address binary Visual Question Answering (VQA) on abstract scenes. We formulate this problem as visual verification of concepts inquired in the questions. Specifically, we convert the question to a tuple that concisely summarizes the visual concept to be detected in the image. If the concept can be found in the image, the answer to the question is "yes", and otherwise "no". Abstract scenes play two roles (1) They allow us to focus on the high-level semantics of the VQA task as opposed to the low-level recognition problems, and perhaps more importantly, (2) They provide us the modality to balance the dataset such that language priors are controlled, and the role of vision is essential. In particular, we collect fine-grained pairs of scenes for every question, such that the answer to the question is "yes" for one scene, and "no" for the other for the exact same question. Indeed, language priors alone do not perform better than chance on our balanced dataset. Moreover, our proposed approach matches the performance of a state-of-the-art VQA approach on the unbalanced dataset, and outperforms it on the balanced dataset.

==> results.tex <==
\section{Results}
\label{sec:results}
%These are the results we are hoping to have in the paper.

\subsection{All approaches we compare to}
\subsubsection*{Without Images}
\begin{itemize}
  \item	All yes as answers  \emph{All-yes}
  \item Train MLP with questions and answers only -LSTM, word2vec, bag-of-words, (maybe sent2vec, skip-thought) call it  \emph{MLP-Q-BOW},  \emph{MLP-Q-Word2Vec}, etc.?
  \item Train MLP with extracted tuples and answers only - word2vec, bag-of-words, (maybe sent2vec, skip-thought) call it  \emph{MLP-T-BOW},  \emph{MLP-T-Word2Vec}, etc.?
  %\item Train above with MLP instead of SVM.
\end{itemize}
\subsubsection*{With Images}
\begin{itemize}
\item Train MLP with questions and answers and images (for text part, just use best feature from above) \emph{MLP-Q+I}
\item Train MLP with extracted tuples and answers and images \emph{MLP-T+I}
%\item Train LSTM with questions with images and answers \emph{LSTM-Q+I}, \emph{LSTM-Q+I}

\item On text side, extract text features(word2vec or bag-of-words) on each PRS arguments for each tuple. On image side, extract image features with emphasize on P and S. Then, reasoning the consistence between them.
%\item On text side, concatenate LSTM with word2vec feature for tuple + image
\item On text side, extract LSTM feature based on the whole questions. On image side, extract image features with emphasize on P and S and reason the consistence.
\item Across all the approaches, we would like to show text+image always has better performance than text alone.
\item The last two are our proposed approaches, compared to ones that use LSTM for question, generic image features fort the whole image, our performance with emphasize on PS has better performance.



\end{itemize}

\subsection{Experiments on balanced dataset}

\begin{itemize}
\item First show language-only models perform similar to chance on the new balanced dataset.

\item A graph-- on x-axis - start from imbalanced dataset, keep on balancing the dataset. On y-axis- language-only models accuracy decreases, our approach accuracy increases or maybe decreases but a little. 

\item We show how well our approach does, train and test on balanced vs. not. Statement about findings.
\item Show that it is not just the more data that helped.

\end{itemize}

\subsection{Analysis}

\begin{itemize}

\item Model is interpretable. Can show which regions of the image it is attending to, in order to generate answer. 

\item Results where we move objects around, remove them, etc. to see when model changes the answer. Enumerate over all existence features. Turn them on/off (flip them). Forward propagate. Measure change in belief of yes. Plot histogram showing which one matters most. 

\item Take advantage of captions to get better models for proposed approach
\item Show question generation

\end{itemize}


==> space_saver.tex <==
% Some illegal space-saving macros
\parskip=3pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
%\renewcommand{\baselinestretch}{0.98} % VERY powerful and VERY illegal. Use carefully

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}

\newlength{\eqnReduceTop}
\newlength{\eqnReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}


%
\setlength{\subsectionReduceTop}{-0.09in}
\setlength{\subsectionReduceBot}{-0.06in}
\setlength{\sectionReduceTop}{-0.08in}
\setlength{\sectionReduceBot}{-0.08in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.05in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\eqnReduceTop}{-0.05in}
\setlength{\eqnReduceBot}{-0.05in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.14in}
\setlength{\captionReduceBot}{-0.12in}
%\setlength{\captionReduceBot}{-0.15in}

